Machine Learning the Disorder Landscape of Majorana Nanowires

We develop a practical machine learning approach to determine the disorder landscape of Majorana nanowires by using training of the conductance matrix and inverting the conductance data in order to obtain the disorder details in the system. The inversion carried out through machine learning using different disorder parametrizations turns out to be unique in the sense that any input tunnel conductance as a function of chemical potential and Zeeman energy can indeed be inverted to provide the correct disorder landscape. Our work opens up a qualitatively new direction of directly determining the topological invariant and the Majorana wave-function structure corresponding to a transport profile of a device using simulations that quantitatively match the specific conductance profile. In addition, this also opens up the possibility for optimizing Majorana systems by figuring out the (generally unknown) underlying disorder only through the conductance data. An accurate estimate of the applicable spin-orbit coupling in the system can also be obtained within the same scheme.

==> Delete/tmain.tex <==

    \title{Machine learning Majorana nanowire disorder landscape}
    \author{Jacob R. Taylor}
    \author{Jay D. Sau}
    \author{Sankar Das Sarma}
    \affiliation{Condensed Matter Theory Center and Joint Quantum Institute, Department of Physics, University of Maryland, College Park, Maryland 20742-4111 USA}
\begin{abstract}
We develop a practical machine learning approach to determine the disorder landscape of Majorana nanowires by using training of the conductance matrix and inverting the conductance data in order to obtain the disorder details in the system.  The inversion carried out through machine learning using different disorder parametrizations turns out to be unique in the sense that any input tunnel conductance as a function of chemical potential and Zeeman energy can indeed be inverted to provide the correct disorder landscape.  Our work opens up a qualitatively new direction of directly determining the topological invariant and the Majorana wave-function structure corresponding to a transport profile of a device using simulations that quantitatively match the specific conductance profile. In addition, this also opens up the possibility for optimizing Majorana systems by figuring out the (generally unknown) underlying disorder only through the conductance data.  An accurate estimate of the applicable spin-orbit coupling in the system can also be obtained within the same scheme.
\end{abstract}
\maketitle 
\begin{bibunit}
\textit{Introduction.\textemdash }
Hybrid superconductor-semiconductor (SC-SM) nanowire structures are the most extensively studied systems for creating laboratory Majorana zero modes (MZMs), which are localized non-Abelian excitations that can be used for creating a topological quantum computer. \cite{aghaee2023inas,das2023search,sarma2015majorana}.  A recent experiment \cite{aghaee2023inas} has provided extensive tunnel conductance measurements to make the case for the existence of small and fragile topological regimes where MZMs should exist at the wire ends.  Earlier experiments in such nanowires were strongly adversely affected by unintentional disorder in the system with the MZM-like conductance signatures arising from disorder-induced trivial Andreev bound states (and not from topological MZMs).  \cite{zhang2021large,das2023search,ahn2021estimating,woods2021charge,pan2021quantized,sarma2021disorder,pan2021three,pan2020physical}  Although cleaner samples are used in \cite{aghaee2023inas},  the disorder situation even for this latest experiment is not yet completely clarified, but the small fragile gaps reported in \cite{aghaee2023inas} indicate that random disorder is likely still playing a role. \cite{sarma2023density,sarma2023spectral}  Disorder has thus emerged as the single most important physical mechanism suppressing topology, certainly in Majorana nanowires, but likely in most solid state topological platforms.  Although the possible importance of disorder in suppressing MZM physics was pointed out early \cite{motrunich2001griffiths,lobos2012interplay,akhmerov2011quantized,liu2012zero,adagideli2014effects,bagrets2012class,takei2013soft,brouwer2011probability,rieder2013reentrant,pikulin2012zero,sau2013density,sau2012experimental}, we still do not have any direct information about the disorder in actual samples, hindering progress in the field.  Understanding and controlling unintentional (and thus, unknown) random disorder has become by far the most important problem in the search for MZMs in solid state platforms. \cite{das2023search} Progress toward the realization of topological MZMs necessitates an understanding of the underlying disorder leading to cleaner and better samples. [\cite{das2023search,sarma2023density,sarma2023spectral}. This leads to the other key problem in the field of identifying MZMs in a device based on its transport characterization. This is because, as already mentioned, the unknown disorder leads to transport signatures that are often misinterpreted as 
MZMs, which often exist in a very limited part of parameter space in moderately disordered devices~\cite{adagideli2014effects,sarma2023spectral}. Ultimately, this motivates the other key challenge in the field, which is to identify when an SC-SM nanowire device has been tuned to support MZMs.

In the current work, we introduce an intuitively appealing Machine Learning (ML) approach for figuring out and understanding the disorder landscape in Majorana nanowires using the tunnel conductance data, which are the standard measurements for Majorana nanowires carried out in every experiment (and simulated in the corresponding theories). 
The disorder potential together with other parameters can then be used to quantitatively verify the validity of the model, which in turn can be used to determine if the transport signature indicates a topological superconducting device. The idea is deceptively simple:  The tunnel conductance depends crucially on disorder, and therefore, it should be possible to invert the measured conductance to extract the underlying disorder.  Of course, the uniqueness of such an inverse scattering problem is a key question since, in principle, it is possible for different disorder landscapes to give similar conductance data.  We solve the uniqueness problem a posteriori by showing that input disorder producing the conductance agrees with the output disorder obtained from our ML procedure.  Our ML approach is powerful, and can be used to obtain other quantities entering the MZM physics, and we estimate the applicable spin-orbit coupling (a key parameter directly determining the nanowire topological gap) using our theory. As a matter of principle, the approach we use can be extended to improve estimates of other parameters of the model. The transport profile of such a complete model can be used to verify the model and provide the most direct correspondence so far of whether the specific transport profile corresponds to a topological device. We mention that other types of ML approaches have been used for optimizing gate operations in Majorana nanowires \cite{thamm2023machine}, but our work is totally different since we use ML to solve the inverse scattering problem of extracting the disorder by using tunnel conductance itself as our training data. More significantly, our ML approach, by providing the unknown parameters for the system, enables a direct realistic estimate for the topological invariant as a function of system parameters to decisively ascertain where the system is topological with MZMs and where it is trivial with no topological properties.  This eliminates all subjective judgments about the topological nature of the system as ML itself provides an answer provided sufficient data are used for the training.



\textit{Theory.\textemdash } We use the extensively used minimal 1D model for Majorana nanowires where the system Hamiltonian is given by a 1D BdG equation and the minimal input parameters are the effective mass (m), the spin-orbit coupling ($\alpha$), the Lande g-factor (g), the parent SC gap,  the SC-SM coupling, the self-consistent chemical potential $\mu$, the magnetic field B, and the disorder potential $V_\text{dis} (x)$.  We follow Ref. \cite{sarma2023spectral} where the details (which are standard in the literature to study SC-SM Majorana nanowires~\cite{sarma2015majorana,pan2021three}) can be found.  Note that all quantities other than $V_\text{dis}$ and $\alpha$ are taken to be fixed and known although this constraint can be relaxed in future works (at the cost of needing much more data for training since more unknown parameters there are, larger must be the training data set).  We use, following Ref.~\cite{aghaee2023inas}, a 3 micron long wire for all our results and discretize the BdG equation using a lattice size of 10 nm as in Ref. \cite{sarma2023spectral}.  We provide the details for the theory and the model in the Supplementary Information (S-1 in SI).

Among these SC-SM nanowire parameters, the specific spatial dependence of the disorder potential $V_\text{dis}(x)$ is completely uncontrolled and  varies among devices as well as slowly over time in the same device. In addition, some system parameters such as $\alpha$ depend on the inversion symmetry breaking of the final device structure, which in general is unknown (and most likely varies from device to device). Given a $V_\text{dis} (x)$, we can solve the BdG equation and generate the 4-component tunnel conductance matrix using the KWANT scattering matrix approach. \cite{groth2014kwant}  In addition, we use the spin-orbit (SO) coupling $\alpha$ also as an unknown parameter.  We vary the disorder potential and $\alpha$ to generate, using KWANT, training transport data (i.e. the 4-component conductance matrix G as a function of the magnetic field $B$ and the chemical potential $\mu$) set for our ML algorithm. We provide details of how the conductance matrix $G$ is computed as a function of $B,\mu$ and other parameters in S-1 of SI. The ML algorithm then predicts $V_\text{dis}$ and $\alpha$ that can be used using KWANT to reproduce a test transport data set. Ideally, in the test transport data would come from experiments. In our proof of principle
demonstration, our test transport data is generated using KWANT with a random choice of $V_\text{dis}(x)$ and $\alpha$. The real test of our ML success is whether the conductance generated using the output $V_\text{dis}(x)$ and $\alpha$ is close to the test transport data set.
%input and output $V_\text{dis}(x)$ and $\alpha$ agree or not.



\textit{Method.\textemdash } Our machine learning model consists of a recurrent neural
network (RNN) created by the package Keras \cite{chollet2015keras} which builds upon tensorflow \cite{tensorflow2015-whitepaper}. In our specific RNN (Fig. 1) each
input step consists of a measurement operation, 7 parameters
consisting of a row of X (4 parameters), which are the components of the conductance matrix $G_{\alpha\beta=L,R}$ and of K (3
parameters), which are the parameters bias voltage $V_{bias}$, chemical potential $\mu$ and magnetic field $B$. 
%and the left and right tunnel barrier voltages $V^{L,R}_{Barrier}$.
The 5 Fourier components of $V_{dis}(x)$ and $\alpha$ are organized into the output vector $Y$ of the RNN in Fig. 1. As described in S-1 of SI, the conductance matrix $X$ is generated for each instance of $K$ and $Y$ using a KWANT simulation. Later we will also discuss data where we use a $10$ Fourier component model for the disorder. In this case $Y$ would be a 11 component vector. For the purpose of ML, it is useful to organize the measurement data into a
combined measurement result matrix $m = [X,K]$. The RNN
is used so that the addition of more measurements would
not decrease the ability of the previous measurements to perform
predictions for a fixed amount of training data. We note that while our RNN is 
sufficient to provide a proof of principle, but can certainly be enhanced/expanded 
in the future by using more elaborate convolutional neural networks, as needed.
In particular the RNN for the case of 5 disorder components 
%5 disorder components and 1 $\alpha$ (5 component model) 
contains 3 GRU hidden recurrent
layers with 150 nodes each, which are then followed up with
a non-recurrent 100 node dense hidden layer. For the
10 component model we instead use 5 GRU layers, still with
150 nodes each.  (More ML technical details are given in \Ref{S:ML} in SI.)

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{NNDiagram.png}
         \caption{}
         \label{fig:1a}
     \end{subfigure}
     \caption{(a) Diagram of the neural network. The machine learning model consists of a recurrent neural network (RNN) portion followed by a dense layer. The RNN for the 5+1 (10) component model consisted 3 (5) GRU hidden recurrent layers with 150 nodes each, followed by a dense hidden layer with 100 nodes. $m_i$ is the $i^\text{th}$ row of $\textbf{m}$, $o_n$ is the final GRU output after $n$ iterations, where $n$ is the total number of rows within $\textbf{m}$. $h_i$ is the state vector after $i$ iterations of GRU. For the 5+1 component model the final output  $Y$ contains $\alpha$ while for the 10 component model it's just the Fourier components of disorder.}
     \label{fig:NNDiagram}
\end{figure}


\begin{figure*}[!htbp]
     \centering
     \begin{subfigure}[b]{0.46\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults//Ex2Gs5_dr=0V.png}
         \caption{}
         \label{fig:2c}
     \end{subfigure}
          \begin{subfigure}[b]{0.46\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults//Ex2Gs5_dr=1V.png}
         \caption{}
         \label{fig:2d}
     \end{subfigure}
          \begin{subfigure}[b]{0.46\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Ex2Gs5_dr=2V.png}
         \caption{}
         \label{fig:2e}
     \end{subfigure}
          \begin{subfigure}[b]{0.46\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults//Ex2Gs5_dr=3V.png}
         \caption{}
         \label{fig:2f}
     \end{subfigure}
     \caption{Representative samples of 5 disorder potential components and $\alpha$ neural network test input and predictions. In (a-d) the first row is $G_{LL}$, $G_{RR}$, $G_{LR}$ and $G_{RL}$ conductance simulations expected for the input disorder potential, and the second row is the calculated conductance measurements for the corresponding predicted disorder potential. Each of (a-d) is for different disorder potential and $\alpha$ realizations (shown in Fig.\ref{fig:D1}). The topological invariant corresponding to this profile can be seen in Fig \ref{fig:VIT1}. The conductance simulations are plotted for different values of $V_{\text{Bias}}$ (in meV) and $B_x$ (in T). These are plotted for $\mu=0$}
     \label{fig:VB1}
\end{figure*}





\begin{figure}[H]
     \centering
      \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/YFourier5.pdf}
         \caption{}
         \label{fig:3a}
     \end{subfigure}
      \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Y5.pdf}
         \caption{}
         \label{fig:3b}
     \end{subfigure}
     \caption{Representative samples of 5 disorder potential components neural network test input and predictions. (a) The discrete cosine transformed components of the disorder potential for 4 different samples and their respective predictions. (b) Disorder potentials in real space with deterministic modification due to boundary effects. The topological invariant corresponding to this profile can be seen in Fig \ref{fig:VIT1}. The disorder amplitude and correlation length for each realization was 1.5meV and 3 sites respectively. Input and output are virtually indistinguishable demonstrating the efficacy of the ML.
     \label{fig:D1}
     }
\end{figure}

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/AlphaCompare.pdf}
         \caption{}
         %\label{fig:1a}
     \end{subfigure}
     \caption{Representative samples of $\alpha$ neural network test input and predictions. The blue points representing the input $\alpha$ values (in meV/nm) and the orange represent the predicted $\alpha$ values.}
     \label{fig:AlphaCompare}
\end{figure}

\begin{figure*}[h!]
     \centering
        \begin{subfigure}[b]{0.95\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/YFourier10.png}
         \caption{}
         \label{fig:5a}
     \end{subfigure}
          \begin{subfigure}[b]{0.95\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Y10.png}
         \caption{}
         \label{fig:5b}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=0V.png}
         \caption{}
         \label{fig:5c}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=1V.png}
         \caption{}
         \label{fig:5d}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=2V.png}
         \caption{}
         \label{fig:5e}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=3V.png}
         \caption{}
         \label{fig:5f}
     \end{subfigure}
     \caption{Representative samples of 10 disorder potential components neural network test input and predictions. (a) The discrete cosine transformed components of the disorder potential for 4 different samples and their respective predictions. (b) Disorder potentials in real space with deterministic modification due to boundary effects. Representative samples of 10 disorder potential components neural network test input and predictions. In (c-f) the first row is $G_{LL}$, $G_{RR}$, $G_{LR}$ and $G_{RL}$ conductance measurements expected from a input disorder potential, and the second row is conductance measurements from the corresponding predicted disorder potential. Each of (c-f) are different disorder potential realizations, shown in (a). The conductance measurements are plotted for different values of $V_{\text{Bias}}$ (in meV) and $B_x$ (in T).   For this model $\alpha=8 meV/nm$ is fixed. The topological invariant corresponding to this profile can be seen in Fig \ref{fig:VIT2}. The disorder amplitude and correlation length for each realization was $1.5$meV and 3 sites respectively. These are plotted for $\mu=0$.}
     \label{fig:dVB2}
\end{figure*}
\textit{Results.\textemdash } We use both  5-component and  10-component representations for our Gaussian random disorder, obtaining very similar results. We measure the ML effectiveness using the standard scaled $R_2$ fidelity parameter between the $Y_{test}$ and $Y_{predicted}$ predicted by the trained RNN. The standard scaling converts the data used in the training processes into a zero mean, unit variance form. $R_2 = 1$ implies perfect prediction, while $R_2 = 0$ is equivalent to just taking the average output of the testing data, ie., no prediction. This scaling and $R_2$ can be found in details on the package scikit-learn \cite{pedregosa2011scikit}.

To train the model for 5 disorder components we generate a total of 8000
$Y$ realizations for a fixed disorder strength.  We split our data such that 90\% is used in the training process and the remaining 10\% used for testing. Using the 800 test realizations we achieve a standard scaled $R_2$ = 0.98, which is an excellent fidelity.  For this model we find it sufficient to use only the zero bias conductance data (i.e. set $V_{bias}=0$ in $K$) to obtain the $98\%$ fidelity already. We emphasize that the ML algorithm predicts $V_\text{dis}$, $\alpha$ accurately enough that they predicted values can be used in KWANT to match a test conductance quite accurately as seen in Fig.~\ref{fig:VB1}. The good $R_2$ value of the predictions of the RNN are apparent from comparing the test and predicted Fourier components of disorder and SO coupling seen in Figs.~\ref{fig:D1} and ~\ref{fig:AlphaCompare}.
%Some representative results are provided in Figs. 2-4, depicting the input and the predicted results for disorder, conductance, and SO coupling. 
(More results are given in the \ref{S:Add} in the SI.) The accuracy of the predicted parameters implies that the $Y$ values predicted by the RNN can also be used to generate the topological invariant in parameter (i.e. $K$) space. To test this we compared the topological visibility in $B-\mu$ space between 
a test case and predicted case and found good agreement as seen in Figs.~\ref{fig:VIT1}~\ref{fig:VIT2}~\ref{fig:VIT} in the SI.

In Fig. 5, we show the results of our 10-component disorder ML results. To train for 10 disorder components we generate a total of 20000 disorder realizations, 90\% of which is used in the training process and the remaining 10\% used to test. We use a fixed $\alpha = 8.0 meV/nm$. Using the 2000 test realizations we achieve a standard scaled $R_2 = 0.79$, which is respectable, but can be improved with more data sets. Due to computational limitations we only use $V_\text{Bias} = 0$ and $V_\text{Bias} = 0.032$ meV (using more values of $V_\text{Bias}$ should increase $R_2$). This lower fidelity is likely due to the need for more training and a larger $K$ matrix since differentiating among 10 component potentials is a more computationally challenging task. Representative results are shown in Fig. \ref{fig:dVB2}, and again, visual inspection shows excellent agreement between the input/output data, verifying the success of our ML approach. 



\textit{Conclusion.\textemdash }We introduce a Machine Learning approach to extract unknown system parameters, particularly the disorder landscape, from the simulated (or measured) tunnel conductance data in hybrid SC-SM Majorana nanowire structures.  We validate the approach by using simulated conductance data as the training set, establishing that such training leads to strongly predictive results for both disorder and spin-orbit coupling using as few as 3 parameters (i.e. $K$) for the  conductance data used in our simulations. The accuracy of the predicted results can be verified by comparing the predicted conductance as well as  topological visibility profiles to the test profiles. The predicted profiles, which are functions of multiple parameters such as $V_{bias}$ and $\mu$ are generated by KWANT from the parameters that are predicted by ML to match a given test conductance data. The topological visibility profile as a function of 
 $B$ and $\mu$ is also generated by KWANT for test conductance data generated by KWANT.  Using experimental conductance data (and a bigger computer), one should be able to generalize our approach to obtain all the relevant parameters for Majorana nanowires, not only the disorder and the SO coupling as we do, but also the g-factor, the SC gap, the number of occupied subbands, etc. since our ML approach is general, and only requires as inputs sufficient amount of conductance training data which are easy to obtain both experimentally and theoretically. Our method, given enough training data and computing resources,  should in principle be able to decisively indicate, just through our ML protocol,  whether a set of conductance data in a particular sample indicates an underlying topological (or trivial) system with MZMs (or not). In particular, by determining all the relevant unknowns, one can simulate a device and calculate its topological invariant directly using the output parameters, decisively indicating whether the sample is or is not topological. 

\section{Acknowledgement}
We thank Maissam Barkeshli for teaching a machine learning course which helped us in developing our approach presented in this paper.  This work is supported by the Laboratory for Physical Sciences.


\putbib
\end{bibunit}
%\input{Sup.tex}

